Rigidification of dendroidal infinity-operads

We give an explicit description of the rigidification of an $\infty$-operad as a simplicial operad. This description is based on the notion of dendroidal necklace, extending work of Dugger and Spivak from the categorical context to the operadic context, although with a different framework, which relates constructions involving necklaces to a standard factorization of maps in the category of trees.

==> xxAC.tex <==



==> xxOC.tex <==



==> xxTAS.tex <==


